Model predictions of wave overwash extent into the marginal ice zone

A model of the extent of wave driven overwash into fields of sea ice floes is proposed. The extent model builds on previous work modelling wave overwash of a single floe by regular waves by including irregular incoming waves and random floe fields. The model is validated against a laboratory experiment. It is then used to study the extent of wave overwash into marginal ice zones consisting of pancake and fragmented floe fields. The effects of wave conditions and floe geometry on predicted extents are investigated. Finally, the model is used to predict the wave overwash extent for the conditions observed during a winter (July) 2017 Antarctic voyage in which the sea surface was monitored by a stereo-camera system.

==> annotations-luke.tex <==
\ifdefined\shownewold
   \newcommand{\del}[1]{{\color{red}\sout{#1}}}
\else
   \newcommand{\del}[1]{\ignorespaces}
\fi
\ifdefined\shownewold
   \newcommand{\deleqn}[1]{\\\del{\parbox{\textwidth}{#1}}}
\else
   \newcommand{\deleqn}[1]{\ignorespaces}
\fi
\ifdefined\shownewold
   \newcommand{\new}[1]{{\color[rgb]{0,0,1}#1}}
\else
   \newcommand{\new}[1]{#1}
\fi
\ifdefined\shownewold
   \newcommand{\old}[1]{{\color[rgb]{0.5,0.5,0.5}#1}}
\else
   \newcommand{\old}[1]{\ignorespaces}
\fi
\ifdefined\shownewold
   \newcommand{\delref}[1]{\del{\parbox{\figwidth\columnwidth}{#1}}}
\else
   \newcommand{\delref}[1]{\vspace{-12pt}}
\fi
\ifdefined\shownewold
   \newcommand{\lu}[1]{{\color[rgb]{1,0,1} #1}}
   \newcommand{\luchange}[2]{\del{#1}\new{#2}}
   \newcommand{\luleft}[1]{{\color[rgb]{1,0,1}$\longleftarrow$#1}}
   \newcommand{\luright}[1]{{\color[rgb]{1,0,1}#1$\longrightarrow$}}
\else
   \newcommand{\lu}[1]{\ignorespaces}
   \newcommand{\luchange}[1]{\ignorespaces}
   \newcommand{\luleft}[1]{\ignorespaces}
   \newcommand{\luright}[1]{\ignorespaces}
\fi
%\ifdefined\shownewold
%   \newcommand{\ma}[1]{{\color[rgb]{0.7,0,0.7} \textit{#1}}}
%\else
%   \newcommand{\ma}[1]{\ignorespaces}
%\fi
%
%%%% COMMENT IN MARGIN \marcomm{comment}[vertical alignment (optional), e.g. -20mm]
%
%\NewDocumentCommand{\marcomm}{mooo}
% {
%  {\normalmarginpar\marginnote[\hspace{#3}{\parbox{#4}{\begin{flushleft}\setstretch{1.0}#1\end{flushleft}}}]{\hspace{#3}{\parbox{#4} {\begin{flushleft}\setstretch{1.0}#1\end{flushleft}}}}[#2] }
%  }
%  
%\NewDocumentCommand{\revmarcomm}{mooo}
% {
%  {\reversemarginpar\marginnote[\hspace{#3}{\parbox{#4}{\begin{flushleft}\setstretch{1.0}#1\end{flushleft}}}]{\hspace{#3}{\parbox{#4}{\begin{flushleft}\setstretch{1.0}#1\end{flushleft}}}}[#2] }
%}  
% 
%\ifdefined\showcomments 
%\NewDocumentCommand{\mymarcomm}{mooo}
%  % #1 = text 
%  % #2 = vertical offset (optional)
%  % #3 = width (optional)
%  % #4 = horizontal offset (optional)
% {
%  \IfValueTF{#4}
%   {\revmarcomm{#1}[#2][#4][#3]}
%    {\IfValueTF{#3}
%     {\revmarcomm{#1}[#2][70pt][#3]}
%      {\IfValueTF{#2}
%       {\revmarcomm{#1}[#2][-0pt][70pt]}
%        {\revmarcomm{#1}[10pt][-0pt][70pt]}
%  }}}
%\else
%   \newcommand{\mymarcomm}[1]{\ignorespaces}
%\fi
  

%\NewDocumentCommand{\mymarcomm}{mo}
% {
% \iffullversion % for either full version
%  \IfValueTF{#2}
%  {\revmarcomm{#1}[#2][-80pt][95pt]}
%  {\revmarcomm{#1}[10pt][-80pt][95pt]}
% \else
% \IfValueTF{#2}
%  {\revmarcomm{}[#2][-80pt][95pt]}
%  {\revmarcomm{}[10pt][-80pt][95pt]}
%  \fi
%  }  

==> colours-luke.tex <==
% COLOURS
%\renewcommand{\white}{\color[rgb]{1,1,1}}
%\newcommand{\lightblue}{\color[rgb]{0,0.5,1}}
%\newcommand{\darkorange}{\color[rgb]{1,0.55,0}}
%\newcommand{\midgreen}{\color[rgb]{0,0.8,0.2}}
%\newcommand{\purple}{\color[rgb]{0.5,0,0.5}}
%\renewcommand{\magenta}{\color[rgb]{1,0,1}}
%\renewcommand{\blue}{\color[rgb]{0,0,1}}
%\renewcommand{\red}{\color[rgb]{1,0,0}}
%\renewcommand{\black}{\color[rgb]{0,0,0}}
%\newcommand{\maroon}{\color[rgb]{0.5,0,0}}
%\newcommand{\teal}{\color[rgb]{0,0.5,0.5}}
%\newcommand{\navy}{\color[rgb]{0,0,0.5}}
%\newcommand{\olive}{\color[rgb]{0.5,0.5,0}}
%\newcommand{\darkgreen}{\color[rgb]{0,0.55,0}}
%\newcommand{\midgrey}{\color[rgb]{0.5,0.5,0.5}}
%\newcommand{\darkgrey}{\color[rgb]{0.75,0.75,0.75}}
%\newcommand{\lightgrey}{\color[rgb]{0.25,0.25,0.25}}

\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0,0.55,0}
\definecolor{midgreen}{rgb}{0,0.8,0.2}
\definecolor{magenta}{rgb}{1,0,1}
\definecolor{purple}{rgb}{0.5,0,0.5}
\definecolor{darkorange}{rgb}{1,0.55,0}
\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{olive}{rgb}{0.5,0.5,0}
\definecolor{midgrey}{rgb}{0.5,0.5,0.5}
\definecolor{lightgrey}{rgb}{0.75,0.75,0.75}
\definecolor{matlabblue}{rgb}{0,0.447,0.741}
\definecolor{matlabred}{rgb}{0.85,0.325,0.098}
\definecolor{lightblue}{rgb}{0,0.5,1}
\definecolor{darkgrey}{rgb}{0.25,0.25,0.25}
\definecolor{teal}{rgb}{0,0.5,0.5}
\definecolor{navy}{rgb}{0,0,0.5}
\definecolor{goldenrod}{rgb}{0.85,0.6,0.1}

\definecolor{OWQ_1}{rgb}{0.3467 ,0.5360,0.6907}%
\definecolor{OWQ_2}{rgb}{0.9153 ,0.2816 , 0.2878}%
		
\definecolor{PRSA_1}{rgb}{0.34667,0.53600,0.69067}%
\definecolor{PRSA_2}{rgb}{0.91529,0.28157,0.28784}%
\definecolor{PRSA_3}{rgb}{0.44157,0.74902,0.43216}%
\definecolor{PRSA_4}{rgb}{1.00000,0.59843,0.20000}%


\definecolor{ColMat_1}{rgb}{0.904706,0.191765,0.19882}
\definecolor{ColMat_2}{rgb}{0.294118,0.544706,0.749412}
\definecolor{ColMat_3}{rgb}{0.371765,0.717647,0.361176}
\definecolor{ColMat_4}{rgb}{1,0.548235,0.1}
\definecolor{ColMat_5}{rgb}{0.865,0.811,0.433}
\definecolor{ColMat_6}{rgb}{0.685882,0.403529,0.241176}
\definecolor{ColMat_7}{rgb}{0.971765,0.555294,0.774118}
\definecolor{ColMat_8}{rgb}{0.64,0.64,0.64}


\definecolor{Gray_1}{rgb}{0.7,0.7,0.7}


==> definitions-luke.tex <==
\newcommand{\ie}{i.e.\ }  
%\newcommand{\eg}{e.g.\ } 
%\newcommand{\etal}{et~al.~}  

\newcommand{\cc}{\textrm{c.c.} } 
\newcommand{\hot}{\textrm{h.o.t.} } 

\newcommand{\diag}{\textrm{diag}}
\newcommand{\real}{\textrm{Re}}
\newcommand{\imag}{\textrm{Im}}
\newcommand{\sech}{\mathrm{sech}}
\newcommand{\arccot}{\mathrm{arccot}}
\newcommand{\cosech}{\mathrm{cosech}}
\newcommand{\mn}{\textrm{mn}}
\newcommand{\mx}{\textrm{mx}}
\renewcommand{\exp}{{\rm exp}}
\newcommand{\eig}{{\rm eig}}
\newcommand{\order}{\textrm{O}}
\newcommand{\bfx}{\textbf{x}}
\newcommand{\bfX}{\textbf{X}}
\newcommand{\bfn}{\textbf{n}}

\newcommand{\trans}{\hspace{1pt} ^\mathrm{t} \hspace{-1pt}}

\newcommand{\inv}{\mathrm{inv}}
\newcommand{\der}{\mathrm{d}} 		% Leibniz derivative
\renewcommand{\d}{\,\mathrm{d}} 	% Integral differential
\newcommand{\pt}{\partial}
\newcommand{\E}{\mathbf{E}} % expected value
\newcommand{\Var}{\mathbf{Var}} % variance
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}
% \newcommand{\llangle}{\langle\langle}
% \newcommand{\rrangle}{\rangle\rangle}
\newcommand{\fourier}{\mathcal{F}} % Fourier transform
\newcommand{\fourierinv}{\fourier^{-1}} % Fourier transform
\renewcommand{\Re}{\mathrm{Re}\,}
\renewcommand{\Im}{\mathrm{Im}\,}
\renewcommand{\i}{\mathrm{i}}

% \renewcommand{\iint}{\int \!\!\! \int}
% \renewcommand{\iiint}{\int \!\!\! \int \!\!\! \int}
\newcommand{\wrt}{\,\mathrm{d}}   
\newcommand{\eps}{\varepsilon}    
\newcommand{\ci}{\mathrm{i}}   
\newcommand{\e}{\mathrm{e}}   
\newcommand{\ds}{\displaystyle}   

\usepackage{enumerate}
\usepackage{ dsfont }
%\usepackage{etaremune}
%\usepackage{enumitem}

\usepackage{overpic,rotating}

%\usepackage[colorlinks=false,urlcolor=blue]{hyperref}

\newcommand{\ttt}[1]{\texttt{#1}}
\newcommand{\tn}[1]{\textnormal{#1}}

% MATHS
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}

\newcommand{\pder}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\deriv}[2]{\frac{{\rm d} {#1}}{{\rm d} {#2}}}

\def\D{}
\renewcommand{\D}[2]{\mathchoice
  {\frac{\partial #2}{\partial #1}}% display
  {{\partial #2}/{\partial #1}}% text
  {{\partial #2}/{\partial #1}}% script
  {{\partial #2}/{\partial #1}}% scriptscript
  }
\newcommand{\Dn}[3]{\mathchoice
  {\frac{\partial^{#2} #3}{\partial #1^{#2}}}%
  {{\partial^{#2} #3}/{\partial #1^{#2}}}%
  {{\partial^{#2} #3}/{\partial #1^{#2}}}%
  {{\partial^{#2} #3}/{\partial #1^{#2}}}%
  }
\newcommand{\DD}[2]{\Dn{#1}2{#2}}
\newcommand{\DDD}[2]{\Dn{#1}3{#2}}
\newcommand{\DDDD}[2]{\Dn{#1}4{#2}}
\newcommand{\Dx}[3]{\mathchoice
  {\frac{\partial^2 #3}{\partial #1 \partial #2}}%
  {{\partial^2 #3}/{\partial #1 \partial #2}}%
  {{\partial^2 #3}/{\partial #1 \partial #2}}%
  {{\partial^2 #3}/{\partial #1 \partial #2}}%
  }
\newcommand{\de}[2]{\mathchoice
  {\frac{\mathrm{d} #2}{\mathrm{d} #1}}% display
  {{\mathrm{d} #2}/{\mathrm{d} #1}}% text
  {{\mathrm{d} #2}/{\mathrm{d} #1}}% script
  {{\mathrm{d} #2}/{\mathrm{d} #1}}% scriptscript
  }
\newcommand{\dn}[3]{\mathchoice
  {\frac{\mathrm{d}^{#2} #3}{\mathrm{d} #1^{#2}}}%
  {{\mathrm{d}^{#2} #3}/{\mathrm{d} #1^{#2}}}%
  {{\mathrm{d}^{#2} #3}/{\mathrm{d} #1^{#2}}}%
  {{\mathrm{d}^{#2} #3}/{\mathrm{d} #1^{#2}}}%
  }
\newcommand{\dd}[2]{\dn{#1}2{#2}}
\newcommand{\ddd}[2]{\dn{#1}3{#2}}
\newcommand{\dddd}[2]{\dn{#1}4{#2}}

\newcommand{\grad}{\mathop{\mathrm{grad}}}
\newcommand{\curl}{\mathop{\mathrm{curl}}}
\renewcommand{\div}{\mathop{\mathrm{div}}}

% HORIZ LINE
\newlength{\mylinelength}
\setlength{\mylinelength}{10pt}
\newlength{\mydashlength}
\setlength{\mydashlength}{4pt}
\newlength{\mydashspace}
\setlength{\mydashspace}{2pt}
\newlength{\mychainlengthA}
\setlength{\mychainlengthA}{3pt}
\newlength{\mychainlengthB}
\setlength{\mychainlengthB}{1pt}
\newlength{\mychainspace}
\setlength{\mychainspace}{1.5pt}
\newlength{\mylinethickness}
\setlength{\mylinethickness}{0.8pt}

\newcommand{\hhh}{\noindent\hfil\rule{0.5\textwidth}{.4pt}\hfil}
\newcommand{\myline}[1]{{\parbox{\mylinelength}{#1\rule{\mylinelength}{\mylinethickness}}}}
\newcommand{\mydash}[1]{{\parbox{\mylinelength}{#1\rule{\mydashlength}{\mylinethickness}\hspace{\mydashspace}\rule{\mydashlength}{\mylinethickness}}}}
\newcommand{\mychain}[1]{{\parbox{\mylinelength}{#1\rule{\mychainlengthA}{\mylinethickness}\hspace{\mychainspace}\rule{\mychainlengthB}{\mylinethickness}\hspace{\mychainspace}\rule{\mychainlengthA}{\mylinethickness}}}}


% MATH EQN TEXT
\newcommand{\mathand}{\quad\textnormal{and}\quad}
\newcommand{\mathandR}{\textnormal{and}\quad}  
\newcommand{\mathandL}{\quad\textnormal{and}}  
\newcommand{\mathfor}{\quad\textnormal{for}\quad}
\newcommand{\mathforR}{\textnormal{for}\quad}  
\newcommand{\mathforL}{\quad\textnormal{for}}  
\newcommand{\mathas}{\quad\textnormal{as}\quad}
\newcommand{\mathasR}{\textnormal{as}\quad}  
\newcommand{\mathasL}{\quad\textnormal{as}} 
\newcommand{\mathwhere}{\quad\textnormal{where}\quad}
\newcommand{\mathwhereR}{\textnormal{where}\quad}  
\newcommand{\mathwhereL}{\quad\textnormal{where}} 
\newcommand{\mathX}[1]{\quad\textnormal{#1}\quad}
\newcommand{\mathXR}[1]{\textnormal{#1}\quad}  
\newcommand{\mathXL}[1]{\quad\textnormal{#1}}  

\newcommand{\MATHand}{\qquad\textnormal{and}\qquad}
\newcommand{\MATHandR}{\textnormal{and}\qquad}  
\newcommand{\MATHandL}{\qquad\textnormal{and}}  
\newcommand{\MATHfor}{\qquad\textnormal{for}\qquad}
\newcommand{\MATHforR}{\textnormal{for}\qquad}  
\newcommand{\MATHforL}{\qquad\textnormal{for}}  
\newcommand{\MATHas}{\qquad\textnormal{as}\qquad}
\newcommand{\MATHasR}{\textnormal{as}\qquad}  
\newcommand{\MATHasL}{\qquad\textnormal{as}} 
\newcommand{\MATHwhere}{\qquad\textnormal{where}\qquad}
\newcommand{\MATHwhereR}{\textnormal{where}\qquad}  
\newcommand{\MATHwhereL}{\qquad\textnormal{where}} 
\newcommand{\MATHX}[1]{\qquad\textnormal{#1}\quad}
\newcommand{\MATHXR}[1]{\textnormal{#1}\qquad}  
\newcommand{\MATHXL}[1]{\qquad\textnormal{#1}}   

% TICK+CROSS
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\tickbox}{{ $\Box$ }}
